Multiscale simulation of interacting turbulent and rarefied gas flows in the DSMC framework

A multiscale stochastic-deterministic coupling method is proposed to investigate the complex interactions between turbulent and rarefied gas flows within a unified framework. This method intermittently integrates the general synthetic iterative scheme with the shear stress transport turbulence model into the direct simulation Monte Carlo (DSMC) approach, enabling the simulation of gas flows across the free-molecular, transition, slip, and turbulent regimes. First, the macroscopic synthetic equations, derived directly from DSMC, are coupled with the turbulence model to establish a constitutive relation that incorporates not only turbulent and laminar transport coefficients but also higher-order terms accounting for rarefaction effects. Second, the macroscopic properties, statistically sampled over specific time intervals in DSMC, along with the turbulent properties provided by the turbulence model, serve as initial conditions for solving the macroscopic synthetic equations. Finally, the simulation particles in DSMC are updated based on the macroscopic properties obtained from the synthetic equations. Numerical simulations demonstrate that the proposed method asymptotically converges to either the turbulence model or DSMC results, adaptively adjusting to different flow regimes. Then, this coupling method is applied to simulate an opposing jet surrounded by hypersonic rarefied gas flows, revealing significant variations in surface properties due to the interplay of turbulent and rarefied effects. This study presents an efficient methodology for simulating the complex interplay between rarefied and turbulent flows, establishing a foundational framework for investigating the coupled effects of turbulence, hypersonic conditions, and chemical reactions in rarefied gas dynamics in the future.

==> 4-Opposing_jet.tex <==
\section{Application of the DIG-SST method in Opposing jet}\label{sec:5}

Opposing jet technology has been introduced directly ahead of the aircraft surface to enhance the thermal protection and maneuverability of the aircraft. Numerous experiments have demonstrated that opposing jets can significantly reduce heat loads and drag in supersonic flows~\cite{aso-2003,daso-2009}. %Furthermore, several numerical studies employing turbulence models, such as the $k$-$\omega$ SST model, have further validated their heat and drag reduction capabilities~\cite{ou-2018}. 
%Additionally, the behavior of opposing jets in rarefied environments has been analyzed using the DSMC method~\cite{raeisi-2019}, with the study domain covering altitudes ranging from 60 km to 90 km~\cite{guo-2024}. Microscale jets have also been simulated and validated using hybrid NS-DSMC solvers~\cite{virgile-2022,liuw-2024}; however, these studies focus only on laminar flows and neglect the effects of turbulence. 
Here, the DIG-SST method is employed to comprehensively examine the interaction between turbulent and rarefied flows.

The computational domain is identical to that depicted in Fig.~\ref{fig:blunt_body_largekn}, with the distinction that a 4~mm wide wall boundary located at upstream of the blunt body surface has been replaced by a jet flow boundary. The characteristics of the jet flow are defined based on the pressure ratio, $P_{\text{ratio}}$, which represents the ratio of the jet flow pressure to the post-shock pressure of the free stream, followed by,
\begin{equation}
    P_{\text{ratio}}=\frac{p_{j,0}}{p_{f,s,0}},
\end{equation}
where $p_{j,0}$ is the stagnation pressure of the jet and $p_{f,s,0}$ is the stagnation pressure of the downstream shock, which is calculated based on the relation of the normal shock for free stream properties. Different pressure ratios have been employed to validate the turbulent effect.
The jet has a constant temperature of 250~K and an exit Mach number of 1.

In the DIG-SST method, which incorporates the $k$-$\omega$ SST turbulence model, the initial values of turbulent kinetic energy $k$ and dissipation frequency $\omega$ must be specified. For the incoming free-flow boundary, a turbulence intensity of $I_t = 0.3\%$ and a turbulent to laminar viscosity ratio $\mu_r = 15$ are initialized. At the jet flow boundary, the turbulence intensity is set to $I_t = 3\%$, with a non-dimensional characteristic length $l_t = 0.118$. The values of $k$ and $\omega$ are calculated as $k=1.5I_t(\|\bm{u}\|)^2$ and $\omega=\sqrt{k}/l_t$, respectively. Additionally, the number of particles initially employed in each cell as well as the sample size are the same as previous computational cases.

The opposing jet flow under different conditions at altitudes of 61.5 km and 80 km, corresponding to Knudsen numbers of 0.125 and 0.01, respectively, is analyzed, as summarized in Table~\ref{tab:jetcondition}. When the jet-to-free-stream number density ratio $n_0/n_\infty$ becomes excessively large, the DSMC method faces significant challenges due to its strict limitations on grid resolution and time step, rendering its results unsuitable as a reference. {For example, under a free-stream Mach number of 15 with $\text{Kn}=0.01$ and $P_\text{ratio}=2.5$, the density of the jet is about 370 times larger than the free stream, such that the mean free path is nearly 370 times smaller.} In this section, the results for $P_{\text{ratio}}=2.5$ and $\text{Ma}=5$ are first obtained and compared using the DSMC, DIG, and DIG-SST methods. Subsequently, the interaction of turbulence and rarefaction effects is investigated for supersonic jet flows at $\text{Ma}=15$ and for increased pressure ratio $P_{\text{ratio}}=5$, based on DIG and DIG-SST methods.


\begin{table}[t]
\centering
\footnotesize
\caption{The general setup for opposing jet flow simulations under various conditions is summarized. A \checkmark indicates both affordable computational cost and acceptable results, $\circ$ denotes affordable computational cost but with results lacking turbulence effects, and $\times$ signifies computational cost is prohibitive.}
\begin{tabular}{ccccccccccc}
\hline
\multirow{2}{*}{Height (km)} & \multirow{2}{*}{$\text{Kn} $} & \multirow{2}{*}{$T_\infty$} & \multirow{2}{*}{$T_{\text{jet}}/T_\infty$} & \multirow{2}{*}{Ma} & \multirow{2}{*}{$P_{\text{ratio}}$}&\multirow{2}{*}{$n_{\text{jet}}/n_\infty$} & \multirow{2}{*}{$\text{Re}_\text{jet}$} & \multicolumn{3}{c}{Methodology}                                                   \\ \cline{9-11} 
                        &                               & &                            &                                            &                     &                                            &                                         & DSMC                      & DIG                       & DIG-SST                   \\ \hline
\multirow{3}{*}{61.8}   & \multirow{3}{*}{0.01}         & \multirow{3}{*}{242.1}    & \multirow{3}{*}{1.03}                    & 5                   & 2.5 & 41.76                                      & 925.4                                   & $\circ$ & $\circ$ & \checkmark \\
                        &                               &                             &                                            & 15 &2.5                  & 371.07                                     & 6425.3                                  & $\bm{\times}$             & $\circ$                   & \checkmark \\
                        &                               &                             &                                            & 15  &5                & 742.1                                    & 12850.6                              & $\bm{\times}$             & $\circ$                   & \checkmark \\ \hline
\multirow{3}{*}{80}     & \multirow{3}{*}{0.125}        & \multirow{3}{*}{198.6}    & \multirow{3}{*}{1.26}                    & 5    &2.5               & 34.27                                      & 44.4                                   & \checkmark & \checkmark & \checkmark \\
                        &                               &                             &                                            & 15   &2.5               & 304.5                                     & 394.1                                & $\bm{\times}$             & \checkmark & \checkmark \\
                        &                               &                             &                                            & 15   &5               & 609.0                                     & 788.3                                & $\bm{\times}$             & $\circ$                   & \checkmark \\ \hline
\end{tabular}
\label{tab:jetcondition}
\end{table}

\subsection{Jet flow in small Mach number environment}

\begin{figure}[!t]
    \centering
\includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D125meshDSMC.png}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D01meshDSMC.png}\\
    \caption{The adaptive grids of (left) $\text{Kn}=0.125$ and (right) $\text{Kn}=0.01$ used to generate the reference DSMC data in SPARTA, are applied within a computational domain same as that of the previous blunt body flow case. The time step $\Delta t$, multiplied by the most probable speed, is carefully constrained to remain smaller than the length of the smallest grid cell. }
    \label{fig:DSMC_jetmesh}
\end{figure}

\begin{figure}[p]
    \centering
\includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D125contour.png}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D01contour.png}\\
    \vspace{-8mm}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D0125uxline.pdf}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D01uxline.pdf}\\
    \vspace{-8mm}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D0125rholine.pdf}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D01rholine.pdf}
    \vspace{-5mm}
    \caption{The temperature contour as well as the macroscopic properties extracted along the horizontal central line when $\text{Ma}=5$, $\text{Kn}=0.125$ (left) and $\text{Kn}=0.01$ (right). The temperature contours are obtained and compared by different methods: DSMC (contour in upper half), DIG (lines in upper half) and DIG-SST (contour in lower half).   }
    \label{fig:jetMa5}
\end{figure}

As discussed in the previous section, the cell size near the jet must be significantly smaller than that in the far field to satisfy the grid requirements of the DSMC method. When $\text{Ma}=5$ with $\text{Kn}=0.125$ and $\text{Kn}=0.01$ , given that the local mean free path is inversely proportional to the local number density, the cell size near the jet is approximately 40 times smaller than that in the far field according to Table \ref{tab:jetcondition}. As shown in Fig.~\ref{fig:DSMC_jetmesh}, to efficiently obtain the reference DSMC data, the Cartesian grids in SPARTA are adaptively refined and coarsened based on the local mean free path, and the grid size is strictly maintained below 1/3 of the local mean free path. Note that without the application of adaptive grid techniques, the computational cost for both cases would become prohibitively high. Additionally, the computational domain as well as the grid size applied in DIG and DIG-SST are the same as previous blunt body flow case.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/Ma5Kn0D0125Surface.pdf}
    \includegraphics[width=0.49\textwidth]{figures/Ma5Kn0D01Surface.pdf}\\
    \caption{Surface properties predicted by different methods when $\text{Ma}=5$, $\text{Kn}=0.125$ (left) and $\text{Kn}=0.01$ (right).}
    \label{fig:Ma5surfacecompare}
\end{figure}
Figure \ref{fig:jetMa5} compares the macroscopic field obtained by the DSMC, DIG and DIG-SST methods. When $\text{Kn} = 0.125$, the Reynolds number is relatively low, the turbulent viscosity predicted by the $k$-$\omega$ SST turbulence model is negligible. Under this condition, the numerical results from the DIG-SST method closely match those of the DIG method, which itself recovers to the original DSMC method due to the relatively high Knudsen number. However, as the Knudsen number decreases to $\text{Kn} = 0.01$, the Reynolds number increases, and the turbulent viscosity predicted by the $k$-$\omega$ SST model becomes significant. In this case, the macroscopic field predicted by the DIG-SST method deviates notably from the DIG and DSMC results, while the DIG and DSMC methods remain in close agreement. The same phenomenon occurs in the prediction of the surface quantities. Figure \ref{fig:Ma5surfacecompare} illustrates the surface pressure and heat flux distributions for different Knudsen numbers. At $\text{Kn} = 0.125$, the predictions from all methods are in good agreement, primarily due to the dominant rarefaction effects. However, at $\text{Kn} = 0.01$, the influence of turbulence becomes significant, leading to slight deviations in surface pressure predicted by the DIG-SST method compared to the other two methods. As the surface heat flux in this case is relatively low, the differences in predictions by the DIG-SST method, while present, remain less pronounced.



\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D125muturbmur.png}
    \includegraphics[width=0.49\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma5Kn0D01muturbmur.png}\\
    \caption{Contour of turbulent viscosity $\mu_{turb}$ (top half) and the ratio of the turbulent to laminar viscosity $\mu_{r}$ from DIG-SST method (lower half) when $\text{Ma}=5$. For $\text{Kn}=0.125$ (left), the turbulent effect is negligible, whereas for $\text{Kn}=0.01$ (right), the primary turbulence arises in the free stream and outer shock regions. }
    \label{fig:Ma5mutur}
\end{figure}
Figure $\ref{fig:Ma5mutur}$ shows the ratio between the turbulent and physical viscosities predicted by DIG-SST when $\text{Ma}=5$. At $\text{Kn}=0.125$,  $\mu_r$ in the shock and jet flow regions ranges from $10^{-4}$ to $10^{-5}$, indicating that the turbulent viscosity $\mu_{turb}$ is negligible compared to the laminar viscosity $\mu_{lam}$ in the rarefied regime. In contrast, at $\text{Kn}=0.01$, the distribution of $\mu_{turb}$ shows a pronounced concentration near the outer shock region, leading to noticeable turbulence effects on the shock position and macroscopic property fields.






\subsection{Jet flow in large Mach number environment}

% The Mach numbers of the free stream are increased to 15 and 30 to investigate the turbulent jet in rarefied environment with the Knudsen numbers remained unchanged. As shown in Table~\ref{tab:jetcondition}, the number density of the jet is very large, leading to the unacceptable computational cost for DSMC method. In this section, the results obtained by DIG and DIG-SST method are compared to investigate the coexist of turbulent and rarefied effects.
To examine the behavior of turbulent jets in rarefied environments, the free-stream Mach numbers are increased to 15, while the Knudsen numbers remain unchanged. As indicated in Table~\ref{tab:jetcondition}, the high number density of the jet results in prohibitive computational costs for the DSMC method. Thus in this section, only the results obtained using the DIG and DIG-SST methods are compared to analyze the interaction between turbulence and rarefaction effects.

\begin{figure}[p]
    \centering
    \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D125rhocontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D01rhocontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15rhostagnationline.pdf}	\\
    \vspace{-2.4mm}
     \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D125Ucontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D01Ucontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15uxstagnationline.pdf}   \\
    \vspace{-2.4mm}
     \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D125Tcontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Ma15Kn0D01Tcontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15Tstagnationline.pdf}  
    \vspace{-8mm}
    \caption{Contours of macroscopic properties for $\text{Ma}=15$ at $\text{Kn}=0.125$ (left column) and $\text{Kn}=0.01$ (middle column) for $P_{\text{ratio}}=2.5$, with results from the DIG method shown in the upper half and DIG-SST in the lower half of each contour. (right column) the corresponding profiles extracted along the horizontal central line. Inset: zoomed-in figures to show the difference in shock and jet region.}
    \label{fig:Ma15macroscopicproperties}
\end{figure}

\begin{figure}[p]
    \centering
    \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Kn0D125Ma15_PR5_rhocontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 10pt 10pt 10pt,clip]{figures/Kn0D01Ma15_PR5_rhocontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15_PR5_stagnationrholine.pdf}	\\
    \vspace{-1mm}
     \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Kn0D125Ma15_PR5_Ucontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Kn0D01Ma15_PR5_Ucontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15_PR5_stagnationUline.pdf}   \\
    \vspace{-2mm}
     \hspace{-8mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Kn0D125Ma15_PR5_Tcontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Kn0D01Ma15_PR5_Tcontour.png}
    \hspace{-11mm}
    \includegraphics[width=0.38\textwidth]{figures/Ma15_PR5_stagnationTline.pdf}  
    \vspace{-6mm}
    \caption{Contours of macroscopic properties for $\text{Ma}=15$ at $\text{Kn}=0.125$ (left column) and $\text{Kn}=0.01$ (middle column) for $P_{\text{ratio}}$=5, with results from the DIG method shown in the upper half and DIG-SST in the lower half of each contour. (right column) the corresponding profiles extracted along the horizontal central line. Inset: zoomed-in figures to show the difference in shock and jet region.}
    \label{fig:Ma15PR5macroscopicproperties}
\end{figure}

Figures~\ref{fig:Ma15macroscopicproperties} presents a comparison of the macroscopic properties field obtained by DIG and DIG-SST methods. As the jet propagates into the flow field, it undergoes rapid expansion and acceleration. This expansion continues until the jet interacts with the free stream, leading to the formation of a distinct Mach disk. The jet flow is compressed and decelerated by the Mach disk, and then adjusts to a state of local equilibrium with the post-shock free stream. This equilibrium results in a lateral deflection of the jet, accompanied by a reverse flow component that reattaches to the surface of the model, completing the flow structure. For $P_\text{ratio}=2.5$, the jet flow is fully turbulent when $\text{Ma}=15$ and $\text{Kn}=0.01$. As shown in Fig.~\ref{fig:Ma15macroscopicproperties}, the Mach disk predicted by DIG-SST shifts slightly closer to the jet region compared to that from DIG. Additionally, the outer shock in the DIG-SST results moves marginally towards the free-stream region compared to the DIG results.  As the Knudsen number increases to 0.125, the enhanced rarefaction effect weakens the outer shock, causing it to become thicker. And in the jet-controlled region, the shape of the Mach disk becomes flatter, as the relatively low Reynolds number of the jet flow diminishes the turbulent effects. Consequently, the macroscopic properties obtained from both the DIG and DIG-SST methods are nearly identical. 

As shown in Fig.~\ref{fig:Ma15PR5macroscopicproperties}, when the pressure ratio $P_\text{ratio}$ increases to 5, compared to $P_\text{ratio}=2.5$,  due to the larger expansion of the jet flow, the Mach disk as well as the outer shock moves towards the free-stream region, while the reattachment point for velocity along the model surface moves towards the outflow region. Since the jet flow is totally turbulent for both $\text{Kn}=0.125$ and $\text{Kn}=0.01$, larger difference occurs for macroscopic properties field obtained by DIG and DIG-SST methods. Moreover, the macroscopic properties extracted along the horizontal centerline are compared in the right column of Fig.~\ref{fig:Ma15PR5macroscopicproperties}. Similarly, the results reveal that coupling with the $k$-$\omega$ SST turbulence model causes the macroscopic properties to change earlier compared to the original DIG method. For instance, compared to the profile obtained using DIG, the temperature profile from DIG-SST starts to rise earlier in the upstream region. Thus, these phenomena demonstrate that the turbulent effects become more pronounced when $P_\text{ratio}=5$, regardless of whether $\text{Kn}=0.125$ or $\text{Kn}=0.01$.




% When $\text{Ma}=15$ and $\text{Kn}=0.01$, where the jet flow is fully turbulent and $P_\text{ratio}=2.5$, the Mach disk predicted by DIG-SST shifts slightly closer to the jet exit compared to that from DIG. Additionally, the outer shock in the DIG-SST results moves marginally towards the free-stream region compared to the DIG results.  As the Knudsen number increases to 0.125, the enhanced rarefaction effect weakens the outer shock, causing it to become thicker. And in the jet-controlled region, the shape of the Mach disk becomes flatter, as the relatively low Reynolds number of the jet flow diminishes the turbulent effects. Consequently, the macroscopic properties obtained from both the DIG and DIG-SST methods are nearly identical. Compared to $P_\text{ratio}=2.5$, when pressure ratio $P_\text{ratio}$ increases to 5, the Mach disk as well as the outer shock moves towards the free-stream region, while the reattachment point for vel

\begin{figure}[!t]
    \centering
    \subfigure[$\text{Kn}=0.125$, $P_{\text{ratio}}=2.5$]{\includegraphics[width=0.49\textwidth,trim=10pt 60pt 10pt 150pt,clip]{figures/Ma15Kn0D125muturbmur.png}}
    \subfigure[$\text{Kn}=0.01$, $P_{\text{ratio}}=2.5$]{\includegraphics[width=0.49\textwidth,trim=10pt 60pt 10pt 150pt,clip]{figures/Ma15Kn0D01muturbmur.png}}\\
    \vspace{-3mm}
    \subfigure[$\text{Kn}=0.125$, $P_{\text{ratio}}=5$]{\includegraphics[width=0.49\textwidth,trim=10pt 60pt 10pt 150pt,clip]{figures/Ma15_PR5_Kn0D125mutrubmur.png}}
    \subfigure[$\text{Kn}=0.01$, $P_{\text{ratio}}=5$]{\includegraphics[width=0.49\textwidth,trim=10pt 60pt 10pt 150pt,clip]{figures/Ma15_PR5_Kn0D01mutrubmur.png}}\\
    \vspace{-3mm}
    \caption{Contours of turbulent viscosity $\mu_{turb}$ (top half) and the ratio of the turbulent to laminar viscosity $\mu_r$ (lower half) obtained by DIG-SST method when $\text{Ma}=15$ under various conditions. The primary turbulence arises between the outer shock the Mach disk.}
    \label{fig:Ma15murmuturb}
\end{figure}



Figure~\ref{fig:Ma15murmuturb} presents the contours of turbulent viscosity $\mu_{turb}$ and the ratio of turbulent to laminar viscosity $\mu_{r}$ obtained using the DIG-SST method for $\text{Ma}=15$ under different conditions. When $\text{Kn}=0.125$ and $P_{\text{ratio}}=2.5$, $\mu_r$ exhibits a small increase in the region between the outer shock and the Mach disk (around $\text{X}=-0.025$ m), while remaining relatively low elsewhere. Consequently, the influence of turbulence in most regions is negligible, and the results closely resemble those obtained with the purely laminar DIG method. However, as the Knudsen number decreases to 0.01, $\mu_r$ becomes significantly larger in the same region, indicating a pronounced turbulent effect, which substantially alters the flow characteristics compared to the laminar case. As the pressure ratio $P_{\text{ratio}}$ increases to 5, the region with the highest $\mu_r$ (around $\text{X}=-0.03$ m) shifts further away from the jet flow region.
However, in both the jet flow and outer shock regions, $\mu_r$ remains significantly elevated, indicating that turbulence plays a more dominant role in these regions compared to lower pressure ratios.




% where the turbulent effect dominates and the ratio $\mu_r$ is extremely large when the Knudsen number decreases to 0.01.


\begin{figure}[!t]
    \centering
    \subfigure[]{\includegraphics[width=0.49\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Ma15surfacepressure.pdf}}
    \subfigure[]{\includegraphics[width=0.49\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Ma15surfaceheat.pdf}}\\
    \vspace{-2mm}
    \subfigure[]{\includegraphics[width=0.49\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Ma15_PR5_surfacepressure.pdf}}
    \subfigure[]{\includegraphics[width=0.49\textwidth,trim=10pt 20pt 10pt 50pt,clip]{figures/Ma15_PR5_surfaceheatflux.pdf}}\\
    \vspace{-2mm}
    \caption{The surface properties obtained by different methods for $P_{\text{ratio}}=2.5$ (upper row) and $P_{\text{ratio}}=5$ (lower row) under different conditions.}
    \label{fig:Ma15surface}
\end{figure}



Figure~\ref{fig:Ma15surface} illustrates the distributions of pressure and heat flux along the blunt body surface. When $\text{Kn}=0.125$ and $P_{\text{ratio}}=2.5$, turbulence effects are relatively weak, and the surface properties obtained using DIG-SST closely resemble those from the DIG method. However, as the Knudsen number decreases to 0.01, the significantly increased jet Reynolds number amplifies the turbulent effect, resulting in an approximately 10\% rise in the peak of surface pressure and heat flux (around $\text{X}=-0.008$ m). With $P_{\text{ratio}}$ increased to 5, the reattachment point shifts toward the outflow region, and accordingly, the peaks of the surface properties also migrate in that direction (around $\text{X}=-0.003$ m). Furthermore, under $\text{Kn}=0.125$, the coexistence of turbulent and rarefied effects leads to surface property values from DIG-SST that are nearly double those predicted by DIG. A similar trend is observed for surface pressure when $\text{Kn}$ decreases to 0.01, with DIG-SST yielding approximately 30\% higher values at the reattachment point. In contrast, at the reattachment point, the angle between the velocity streamlines and the model surface is exceedingly small, indicating that the streamlines are nearly parallel to the surface. 
This phenomena produces an almost zero heat flux at the reattachment point, rendering the predictions from both methods essentially indistinguishable.










